Montsalvat: Partitioning Java Applications to Minimize the TCB in Intel SGX

The popularity of the Java programming language has led to its wide adoption in cloud computing infrastructures. However, Java applications running in untrusted clouds are vulnerable to various forms of privileged attacks. The emergence of trusted execution environments (TEEs) such as Intel SGX mitigates this problem. TEEs protect code and data in secure enclaves inaccessible to untrusted software, including the kernel and hypervisors. To efficiently use TEEs, developers must manually partition their applications into trusted and untrusted parts, in order to reduce the size of the trusted computing base (TCB) and minimise the risks of security vulnerabilities. However, partitioning applications poses two important challenges: (i) ensuring efficient object communication between the partitioned components, and (ii) ensuring the consistency of garbage collection between the parts, especially with memory-managed languages such as Java. We present Montsalvat, a tool which provides a practical and intuitive annotation-based partitioning approach for Java applications destined for secure enclaves. Montsalvat provides an RMI-like mechanism to ensure inter-object communication, as well as consistent garbage collection across the partitioned components. We implement Montsalvat with GraalVM native-image, a tool for compiling Java applications ahead-of-time into standalone native executables that do not require a JVM at runtime. Our extensive evaluation with micro- and macro-benchmarks shows our partitioning approach to boost performance in real-world applications

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


==> architecture.gael.tex <==
%!TEX root = main.tex

\section{Architecture}
\label{sec:architecture}
%\paragraph{Design considerations.}
%The design of \sys introduces two important issues: minimizing the TCB, and maximizing enclave memory. A design approach based on a libOS like SCONE or Graphene SGX introduces thousands of lines of code into the enclave runtime, increasing security risks. Furthermore, with such a design, the enclave quickly reaches its memory limitation leading to a dramatic loss of performance. 


\begin{figure*}[!t]
	\centering
	\includegraphics[scale=0.4]{fig/graalsgx_workflow}
	\caption{Overview of \sys framework. Annotated Java code is compiled to bytecode. The latter is transformed in the bytecode weaver to produce two versions of the application classes which are used by the native image generator for trusted and untrusted image generation. The trusted and untrusted images are linked with enclave libraries in the SGX module to build the final SGX application. \py{to fix/redraw eg with omnigraffle}}
	\label{fig:arch}
\end{figure*}

%\subsection{General overview}
%\label{sec:overview}
%\begin{itemize}
%	\item present the workflow (figure and text): annotated application, transformer, generator, etc.
%	\item Show a synthetic illustrative example. This example should include all use cases that we cover (all annotation types, method calls, parameters, return type, etc. The remaining sections will rely on the example.
%	\item Present our assumptions
%\end{itemize}

The primary goal of \sys is to partition applications for SGX enclaves. 
As such, the final partitioned application results in a \textit{trusted} and \textit{untrusted} part, respectively running inside and outside the enclave.
%This section presents the overall workflow of \sys.
Figure \ref{fig:arch} outlines the complete workflow, from application source code to generation of the final SGX application. 
It comprises 4 main phases: \emph{(1)} code annotation, \emph{(2)} bytecode transformation, \emph{(3)} native image partitioning, and \emph{(4)} SGX application creation. 

To illustrate the inner workings of our framework, we consider a synthetic Java application to be partitioned, shown in Listing~\ref{lst:simple:1}.
There are three classes interacting via method calls with each other: classes \texttt{Account} and \texttt{AccountRegistry} perform sensitive operations, thus should be secured in an enclave. 
Instead, class \texttt{Person} is untrusted.


\begin{lstlisting}[caption={Illustrative example.}, label={lst:simple:1}, basicstyle=\tiny]
@Trusted
public class Account {
	private String owner;
	private int balance;		
	public Account(String name, int bal){
		this.owner = name;
		this.balance = bal;
	}	
	public void updateBalance(int val){
		this.balance += val;
	}
}	
@Trusted
public class AccountRegistry {
private List<Account> reg = new ArrayList<Account>();//Trusted obj within a trusted obj
public AccountRegistry() {}
public void addAccount(Account acc) {
this.reg.add(acc);
}}
@Untrusted
class Person {
	private String name;
	private Account acc;//Trusted obj within a untrusted obj.
	public Person(String name, int bal){
		this.name = name;
		this.acc = new Account(name,bal);	
	}	
	public Account getAccount(){
		return this.acc;
	}	
	public void transfer(Person receiver, int sum){
		receiver.getAccount().updateBalance(sum);
		this.acc.updateBalance(-sum);
}}
\end{lstlisting}


\subsection{Partitioning language}
\label{sec:language}
%\begin{itemize}
%	\item Justify our approach: why code annotation instead of data partitioning (intuitive for the developer). 
%	\item Explain our annotation types
%	\item Use our example to illustrate
%\end{itemize}
When partitioning applications destined for enclaves, an important question which arises is how to specify what should be secured or not. 
Some recent works propose annotation of sensitive data~\cite{glamdring}, others propose annotation of sensitive routines~\cite{uranus,civet}. 
While these strategies work, we argue they are not always very intuitive for an application developer. \gt{Why?}
Furthermore, they require complex and expensive data flow analysis to ensure sensitive data is not leaked. 

Instead, we propose a technique based on \textit{class annotations}. \gt{It means that you annotate sensitive data, while you just said that it's not convenient for the developer:)} \gt{I think that the main difference is that you annotate at a class basis and not at an instance/structure basis? But I don't see why it's a better idea :) ? We can say that instead of relying on a complex data flow analysis, we can leverage the Java type system? But it's an engineering issue: for the developer, it does not bring anything. Only with a data flow analysis, the developer can make mistake because the developer can think that a data is sensitive while, for the data flow analyzer it's not the case. By annotating a class, the developer always know if an object resides inside or outside the enclave }
Classes are a fundamental building block for object oriented applications, and it is very intuitive to reason about security along class boundaries. \gt{See my previous comment: I think that it's not a problem of reasoning, but more that you don't have to reason about your code :) Simply by taking a look at the type of a data or of a field, we can know if the object is trusted/untrusted. It's probably better that a data flow analysis where a developer may make mistakes/create bugs.}
Using annotations, developers can easily specify which class needs to be secured and which class needs not be secured.\gt{+ neutral class => here we have to explain that we have three categories: trusted, untrusted, neutral.}
\sys supports two principal annotations: \texttt{Trusted} and \texttt{Untrusted} which developers can use to specify secured and unsecured classes, respectively. \gt{You have to explain what is under the hood :) Trusted class means that the class holds sensitive data that you want to protect. Untrusted class means that you don't want to see this class in the enclave (but why you would want that? you could put everything in the enclave:). You have the ``other'' classes. Basically, for me, you have just trusted classes. All the other are supposed to reside outside the enclave in order to minimize the TCB (important to recall that here). However, for the developer, only the two categories is a little bit complex because the developer may want to use utility classes that provides common data structures such as ArrayLists, LinkedLists, HashMap etc... For these classes, which we define as utility class.}
In Listing~\ref{lst:simple:1}, \texttt{Account} and \texttt{AccountRegistry} classes are annotated as trusted, while class \texttt{Person} is untrusted.

A \texttt{Trusted} class will always be instantiated and manipulated inside the enclave.
This has two implications.
First, its member fields which are not instances of \texttt{Untrusted} classes will be allocated on enclave's heap\vs{add example from Account}\vs{check if we mention earlier how enclave's heap and untrusted heap are maintained/init}.
Second, its methods are always executed inside the enclave.
Similarly for a class annotated as \texttt{Untrusted}, its objects will be allocated only on the untrusted heap, as well as all its member fields not instances of \texttt{Trusted} classes.
All its methods will be executed outside the enclave.
However, some classes need not be inherently\vs{explicitely?} trusted or untrusted \eg utility classes as \texttt{Arrays}, \texttt{Vector}, \texttt{String} or other application-specific classes.
We refer to these classes as \texttt{Don't-care} classes.
\texttt{Don't-care} classes are not annotated.
\vs{personally i find 'Don't-care' not usefriendly as a term, with a dash and a \''. Could we use Ignored ?}
One may legitimately question the relevance of two annotations, thinking that the annotation \texttt{Trusted} is sufficiently expressive.
We could simply annotate trusted classes and consider unannotated classes as untrusted, to be instantiated out of the enclave.
This naive approach is not tractable because for an application to run inside the enclave, not only application specific trusted classes are needed, but also GraalVM runtime components and associated classes (\eg, the GC).
Considering a solution which keeps these classes out of the enclave is not tractable because of the number of ecall and ocall it will generate.
By explicitely allowing the developper to specify \texttt{Untrusted}, thus \texttt{Don't-care}\vs{Ignored} classes, \sys generates a native image for the enclave which will lead to fewer ecall/ocall.\vs{a reviewer might be believe that this trade-off will shown in the eval}
\sys maintains a single state of a \texttt{Trusted} or an \texttt{Untrusted} object in the two worlds leveraging \texttt{proxy} objects (see \S\ref{sec:byte-code-partitioning}).
This is not the case for \texttt{Don't-care} classes which copies evolve independently in both worlds. 
%\at{Peterson justifies why we need Untrusted annotation and Don't care. If explained below, give some few words which intuitively justify them, and ref the corresponding section. Some thing like this: One may wonder while xxxx.}

\smallskip\noindent\textbf{Assumptions}
We assume all annotated classes are fully encapsulated (\ie class fields are private). 
On the one hand, this prevents complex and expensive data flow analysis to prevent sensitive class fields from leaving the enclave \py{@Gael maybe you can expantiate here a little more :)}. 
On the other hand, it ensures that all class fields can only be accessed from outside classes via public methods \eg getters and setters exposed by the class. 
As such, it is easier to control access to these sensitive class fields by applying techniques such as transparent encryption/decryption at the level of these public methods. 
Encapsulation being one pillar of object orientation, we believe this assumption to be reasonable.

\subsection{Bytecode transformation}
\label{sec:byte-code-partitioning}
%\begin{itemize}
%	\item Partition at the byte code level. Explain why.
%	\item Proxy object creation
%	\item Parameter and return object management
%\end{itemize}
\at{First explain the purpose of this step.}
To better understand the purpose of this phase, we will begin by noting that the final partitioned application consists of two native images: a \textit{trusted} and an \textit{untrusted} image. 
The trusted image will not have any untrusted functionality, and the untrusted image will not have any trusted functionality. 
However, trusted objects (\ie instances of trusted classes) may call untrusted objects (\ie instances of untrusted classes) and vice versa. 
Hence, we need to have a way to access untrusted functionality from the trusted runtime and trusted functionality from the outside. 
To do this, we introduce the notion of \textit{proxy classes}. In the trusted runtime, we will have proxy classes for untrusted classes and in the untrusted runtime we will have untrusted proxy classes for the trusted classes. These proxies will serve as gateways to access the functionality (\ie methods) of the real class in the opposite runtime.The proxy classes expose the same methods as the original class, but do not perform any application specific functions themselves. Instead they perform enclave transitions at to access the real functionality in the opposite runtime. This design makes cross enclave object communication easier and helps maintaining the object oriented nature of the program as a whole after it is partitioned. We do bytecode transformations to create these proxy classes and inject code which will permit to do enclave transitions

For all trusted classes, \sys automatically introduces corresponding proxy classes, and for all untrusted classes, it introduces corresponding untrusted proxy classes. 
%\at{Well explain why we need proxy? Rely on the illustrative example.}
%\at{Do we really have proxies for \underline{all} classes? I don't think so. Clarify. If I remember, we do have proxy object only when there is a mix, a parameter, return type, etc. We should clarify and explain all cases which require a proxy. Rely on the illustrative example. Show the resulting code.}
%To build\at{to build or inject?} proxy classes, we leverage a technique called \textit{bytecode weaving}. The latter involves editing or generating code by modifying compiled .class files directly. Bytecode weaving is more efficient and practical when compared to similar approaches like \textit{source code weaving}~\cite{weaving}.

\at{Show a java version of the bytecode with proxy objects.}
In \sys, the bytecode weaver is responsible for doing these bytecode transformations. For trusted image generation, it creates proxy classes for untrusted classes by stripping the methods of the untrusted classes. The bodies of the stripped methods are replaced with native routines which will perform Ocall transitions to the corresponding method in the untrusted runtime. Analogously, for untrusted image generation, the bytecode weaver creates proxy classes for trusted classes by stripping all methods of trusted classes, and replacing the method bodies with native methods which will perform Ecall transitions. The proxy class fields are removed and an \texttt{id field} is added to each proxy class which stores the hash of the corresponding object. The result of these stripping operations is the removal from the trusted and untrusted runtime of all untrusted and trusted functionality respectively. \texttt{Don't care} classes are not modified.

In the rest of the paper, we refer to all unstripped classes as \textit{concrete classes} and stripped classes as \textit{proxy classes}. We call the instances of these classes \textit{concrete objects} and \textit{proxy objects} respectively. If a concrete object in one runtime (trusted or untrusted) has a correspondence with a proxy object in the opposite runtime, we refer to that concrete object as a \textit{mirror object} (\ie the proxy's mirror copy).

For the illustrative example, class \texttt{Person} will be made a proxy for trusted image generation, while classes \texttt{Account} and \texttt{AccountRegistry} will be made proxies for untrusted image generation.


\smallskip\noindent\textbf{Relay methods.}
For methods in one runtime to be callable from the other runtime, these methods must be exported as \textit{entrypoints}. GraalVM Native Image provides an annotation (\texttt{@CEntryPoint}~\cite{centrypoint}) for specifying entrypoint methods which can be callable from C. These entrypoint methods must be static and may only have non-object parameters and return types \ie primitive types or Word types (including pointers)~\cite{graalSite}. As a result of these restrictions, it is not feasible to export all methods of concrete classes as entrypoints directly, as this will mean making the latter all static with non-object parameters. The solution to this problem is to introduce static entrypoint methods which will act as wrappers for the invocations of the associated class or instance methods. We call these methods \textit{relay methods}. 

For each method in a concrete class, including all constructors, the bytecode weaver adds an associated relay method to the class. The native methods added to the stripped methods of the proxy classes  will perform enclave transitions to invoke the corresponding relay methods.


The parameters of a relay method comprise: the id of the calling proxy object (for non-static methods), all primitive parameters of the associated method, and pointers (~\ie \texttt{CCharPointer}~\cite{ccharpointer}) which represent the addresses of buffers obtained from the serialization of any object parameters which are instances of don't care classes.\py{@Tchana you could expantiate here a little more}. For proxy object parameters, the id of the corresponding proxy is passed as parameter and the corresponding mirror object will be used as the parameter once the real method is called in the opposite runtime. Similarly, for mirror object parameters, the id of the corresponding proxy is also sent, and the corresponding proxy object is used in the opposite runtime as parameter in the method.

In the body of the relay method, serialized buffers are deserialized and the corresponding object parameter recreated. For relay methods of constructors, we add code to instantiate the corresponding mirror object, and code to add the mirror object strong reference - proxy id pair to a global registry, which we call the \textit{mirror-proxy registry}. For instance methods, we add code to look up the corresponding mirror object in the registry, and then invoke the instance method on that mirror object with its corresponding parameters. Don't care object return types from the untrusted runtime are also serialized and copied across the enclave boundary. Both the trusted and untrusted runtimes have a mirror-proxy registry.

For the illustrative example, the proxy class \texttt{Account} will look like this after bytecode weaving:

\begin{lstlisting}[caption={Proxy class Account.}, label={lst:simple}]
public class Account {
private int hash;		
public Account(String name,int bal){
	byte[] buff = serialize(name);
	CCharPointer ptr = getPointer(buff);
	ecall_relay_Account(hash,ptr,bal);
}	
public void updateBalance(int val){
	ecall_relay_updateBalance(this.hash,val);
}}	
\end{lstlisting}

The corresponding relay method (\texttt{ecall\_relay\_Account}) will be woven into concrete class \texttt{Account} in the trusted runtime. The following code outlines the state of concrete class \texttt{Account} after byte weaving.

\begin{lstlisting}[caption={Concrete class Account.}, label={lst:simple}]
public class Account {
private String owner;
private int balance;		
public Account(String name,int bal){...}
public void updateBalance(int val){...}

@CEntryPoint
public static void relay_Account(int hash,CCharPointer buff,int bal){
	String name = deserialize(buff);
	Account mirror = new Account(name,bal);
	mirrorProxyRegistry.add(hash,mirror);
}
@CEntryPoint
public static void relay_udpateBalance(int hash,int val){
	Account mirror = mirrorProxyRegistry.get(hash);
	mirror.updateBalance(val);
}}

\end{lstlisting}

For proxy class \texttt{Person}, we will have Ocalls instead to the relay methods. For proxy class \texttt{AccountRegistry}, we have a proxy \texttt{Account} as parameter in the \texttt{addAccount} method. Only its id will be passed to the opposite runtime. The resulting proxy method will be as follows:

\begin{lstlisting}[label={lst:simple}]
public void addAccount(Account acc){
ecall_relay_addAccount(acc.getHash());
}
\end{lstlisting}

The corresponding relay method in concrete class\\ \texttt{AccountRegistry} will be as follows:
\begin{lstlisting}[label={lst:simple}]
@CEntryPoint
public static void relay_addAccount(int hash){
Account mirror = mirrorProxyRegistry.get(hash);
this.addAccount(mirror);
}
\end{lstlisting}

\smallskip\noindent\textbf{Native transition methods.}
The native transition methods (\eg \texttt{ecall\_addAccount }\etc) are C routines which perform enclave transitions to the opposite runtime. At the time of bytecode transformation, the definitions of the native transition methods are absent and only their signatures are provided. Their definitions will be generated by the native image generator. 

The bytecode weaver is based on Javassist~\cite{jassist}, a popular bytecode instrumentation framework.


\subsection{Native image partitioning}
\label{sec:native-image-partitioning}
%\begin{itemize}
%	\item How we decide which runtime class should be integrated into the enclave native image
%	\item Entry classes
%	\item Isolates?
%	\item sgx wrappers
%\end{itemize}
The GraalVM native image generator is responsible for building native images. It takes as input compiled application classes (bytecode), and all their associated external libraries, including the JDK; we note the set of external libraries as \texttt{L}. The native image generator then performs static analysis to find the reachable program elements (\ie classes, methods and fields) starting from the application entrypoints (\ie \texttt{main} method, and all \texttt{@CEntryPoint} methods). Only the reachable methods from these are ahead-of-time compiled into the final native image. For an SGX-based environment, this is particularly useful as it permits to exclude any redundant application logic from the enclave. The resulting image includes runtime components for garbage collection (memory management), thread scheduling, deoptimization \etc. Substrate VM (SVM) is the collective name for these components in GraalVM. 

The bytecode weaving process produces two sets of class files: the first set (\texttt{T}) comprises modified trusted classes and untrusted proxy classes, while the second set (\texttt{U}) comprises modified untrusted classes and secure proxy classes. The set of 
unannotated/\texttt{Don't-care} classes (\texttt{D}) are not changed by the bytecode weaver. These 3 sets of classes are used by GraalVM to generate two native images which represent the partitioned application.


In \sys, the native image generator uses set ($T\cup D\cup L$) as input for \textit{trusted image} generation and the set ($U\cup D\cup L$) as input for \textit{untrusted image} generation. More specifically the trusted image will comprise all the trusted classes reachable in the application, all the untrusted proxy classes reachable from these trusted classes, and all other classes (external libraries and don't care classes) reachable from these. Similarly, the untrusted image will comprise all the untrusted classes reachable in the application, all the trusted proxy classes reachable from these untrusted classes, and all other classes (external libraries and don't care classes) reachable from these.

We modified GraalVM's default native image builder to generate these two images for each application to be partitioned. 

By default, GraalVM's image generator compiles the methods and links the latter with GraalVM's native libraries to produce an executable or a shared object file. We modified the image generator to bypass the linking phase that produces executables or shared objects, so as to produce relocatable object files (.o) which can be linked to other libraries to build the final SGX application. The resulting images for the trusted and untrusted parts are \texttt{trusted.o} and \texttt{untrusted.o} respectively. These will be dispatched to the SGX module and used to build the final SGX application.


%NB: speculative optimization can be done in a program based on profiling data collected during program execution e.g type specializations for interfaces. If the program invalidates these assumptions at runtime, e.g when a second class implementing the said interface is loaded, deoptimizations will need to be done at the level of the VM 

\smallskip\noindent\textbf{SGX code generator.}
During bytecode weaving, native transition routines (Ecalls and Ocalls) were added to proxy classes. We extended GraalVM's native image builder with a class to generate C code definitions for the corresponding Ecalls (added in trusted proxy classes) or Ocalls (added in untrusted proxy classes), as well as their corresponding header files. This code generator also creates associated EDL files which will be used by the Edger8r tool in the Intel SGX SDK to build bridge routines which will help in marshalling data across the enclave boundary. The generated files are dispatched to the SGX module.



\subsection{SGX application creation}
\label{sec:sgx-app-creation}
This is the final stage in the \sys workflow. The \textit{SGX module} is the component responsible for building the final SGX application based on the generated native images. This module builds SGX applications following the standard Intel SGX SDK application design which requires the application to be divided into trusted and untrusted components. %The trusted components and compiled together to produce the final enclave shared object which is loaded in secure memory at runtime.

Because SGX enclaves operate only in user mode, they cannot issue system calls and standard OS abstractions (e.g., file systems, network), which are ubiquitous in real world applications. The solution to this problem is to relay these unsupported calls to the untrusted runtime, which does not have the same limitations. In contrast to systems which introduce a LibOS into the enclave, we leverage an approach which involves redefining unsupported libc routines as wrappers for ocalls. These redefined libc routines in the enclave constitute the \textit{shim library}. The latter intercepts calls to libc routines and relays them to the untrusted runtime. A \textit{shim helper library} in the untrusted runtime then invokes the real libc routines. This by design reduces the TCB when compared to LibOS-based systems.


The SGX module compiles all generated Ecalls and statically links the latter with the trusted image (\texttt{trusted.o}), the shim library, and native libraries from GraalVM to produce the final enclave shared library which corresponds to the trusted component of the SGX application. Similarly, the generated Ocalls are also compiled and linked with the untrusted image (\texttt{untrusted.o}) and GraalVM native libraries to produce the final untrusted component. In accordance with Intel SGX's application model, we compile the main entrypoint of partitioned applications in the untrusted component. The resulting trusted and untrusted components comprise the final SGX application. 

Following our illustrative example, consider the following main routine executing in the untrusted runtime:
\begin{lstlisting}[label={lst:simple}]
public static void main(String[] args) {
	Person p1 = new Person("Alice",100);
	Person p2 = new Person("Bob",25);
	p1.transfer(p2,25);
	AccountRegistry reg = new AccountRegistry();
	reg.addAccount(p1.getAccount());	
}
\end{lstlisting}

During object creating for \texttt{Person} $p1$ and $p2$ their constructors will instantiate a proxy object of the \texttt{proxy Account class}. The String parameters \texttt{"Alice"} and \texttt{"Bob"} will be serialized and an Ecall transition will be made to create a corresponding \texttt{mirror Account object} in the enclave. Similarly, when \texttt{p1.transfer(p2,25)} is called, the corresponding \texttt{proxy Account objects} will perform enclave transitions to update the balances in the enclave. In the same way, the call to \texttt{proxy AccountRegistry} constructor performs a transition to create a mirror object in the enclave corresponding to proxy object \texttt{reg}. The latter performs a transition too when \texttt{addAccount} is called.

\subsection{Garbage collection}
\label{sec:garbage-collection}
%\begin{itemize}
%	\item Two GC
%	\item Describe the GC of each world
%\end{itemize}

Following our partitioned application design, untrusted code objects can have trusted counterparts and vice versa. This presents a challenge at the level of garbage collection because we must ensure synchronized destruction of objects across the trusted and untrusted heaps. More specifically, we need to synchronize GC of proxy and mirror objects; \eg the mirror of proxy object \texttt{reg} should not be destroyed before \texttt{reg}.

To address this problem, we implemented an application level GC helper. When a proxy object is created, we store a weak reference to it in a global list, as well as its id. The GC helper thread periodically scans this list for null weak references. Once such a null weak reference is found, it means the corresponding proxy object has been garbage collected, and thus we can remove the mirror object from the mirror-proxy registry in the opposite runtime. Both the trusted and untrusted runtimes maintain independent lists of proxy weak references for the associated runtime, and two GC helper threads are spawned in the application: one to scan the trusted list in the enclave, and the other to scan the untrusted list. Algorithm \ref{alg:gc-helper} outlines the work of the GC helper thread. 


\begin{algorithm}[th]
	\caption{GC helper thread.}
	\label{alg:gc-helper}
	\begin{algorithmic}[1]
		\State $\mathit{proxyWeakRefs} \gets \{\mathit{list~of~proxy~obj~weak~refs}\}$
		\While {!stopped}
		\State $wait(TIME)$
		\ForAll{$ref\in\mathit{proxyWeakRefs}$}
		\If{$ref = null$}
		\State $\mathit{proxyId} \gets \mathit{getProxyId()}$
		\If{$inEnclave$}
		\State $\mathit{ocall\_removeMirror(proxyId)}$ 					
		\Else
		\State $\mathit{ecall\_removeMirror(proxyId)}$ 
		\EndIf
		\State $\mathit{proxyWeakRefs}\gets \mathit{proxyWeakRefs}\setminus \mathit{ref}$
		\EndIf
		\EndFor
		\EndWhile
	\end{algorithmic}
\end{algorithm}



The \texttt{removeMirror} ocalls or ecalls perform an enclave transition which removes the mirror object - proxy id pair from the corresponding mirror-proxy registry. This automatically makes the mirror object eligible for GC if it is not strongly referenced somewhere else in the program.


\subsection{Running unpartitioned native images in \sys}
Inspite of the benefits of partitioning an enclave application, situations may arise where it is much easier for the application developer to run the entire application as a native image in the enclave. This could happen when the majority of classes potentially deal with sensitive information and no classes qualify as untrusted. For this, we offer the possibility to run the unpartitioned application with \sys. Here no annotations are required and hence no bytecode modifications are done. The original application is built into a single native image which is linked entirely to the final enclave object. Running the entire native image in an enclave increases the TCB but we argue here that the TCB increase is small relative to the same application running on a full-blown JVM in an enclave. Furthermore, the increased heap size due to the entire JVM in the enclave could strain the EPC leading to performance degradations in the application.









==> architecture.tex <==
%!TEX root = main.tex

\section{Architecture}
\label{sec:architecture}
%\paragraph{Design considerations.}
%The design of \sys introduces two important issues: minimizing the TCB, and maximizing enclave memory. A design approach based on a libOS like SCONE or Graphene SGX introduces thousands of lines of code into the enclave runtime, increasing security risks. Furthermore, with such a design, the enclave quickly reaches its memory limitation leading to a dramatic loss of performance. 


\begin{figure*}[!t]
	\centering
	\includegraphics[scale=0.4]{fig/graalsgx_workflow}
	\caption{Overview of \sys framework. Annotated Java code is compiled to bytecode. The latter is transformed in the bytecode weaver to produce two versions of the application classes which are used by the native image generator for trusted and untrusted image generation. The trusted and untrusted images are linked with enclave libraries in the SGX module to build the final SGX application. \py{to fix/redraw eg with omnigraffle}}
	\label{fig:arch}
\end{figure*}

%\subsection{General overview}
%\label{sec:overview}
%\begin{itemize}
%	\item present the workflow (figure and text): annotated application, transformer, generator, etc.
%	\item Show a synthetic illustrative example. This example should include all use cases that we cover (all annotation types, method calls, parameters, return type, etc. The remaining sections will rely on the example.
%	\item Present our assumptions
%\end{itemize}

The primary goal of \sys is to partition Java applications for SGX enclaves. 
As such, the final partitioned application results in a \textit{trusted} and \textit{untrusted} part, respectively running inside and outside the enclave.
%This section presents the overall workflow of \sys.
Figure \ref{fig:arch} outlines the complete workflow, from application source code to generation of the final SGX application. 
It comprises 4 main phases: \emph{(1)} code annotation, \emph{(2)} bytecode transformation, \emph{(3)} native image partitioning, and \emph{(4)} SGX application creation. 

To illustrate the inner workings of our framework, we consider a synthetic Java application to be partitioned, shown in Listing~\ref{lst:simple:1}.
There are three classes interacting via method calls with each other: classes \texttt{Account} and \texttt{AccountRegistry} perform sensitive operations, thus should be secured in an enclave. However, class \texttt{Person} is untrusted, and will not be included in the enclave.


\begin{lstlisting}[caption={Illustrative example.}, label={lst:main}, basicstyle=\tiny]
@Trusted
public class Account {
	private String owner;
	private int balance;		
	public Account(String name, int bal){
		this.owner = name;
		this.balance = bal;
	}	
	public void updateBalance(int val){
		this.balance += val;
	}
}	
@Trusted
public class AccountRegistry {
private List<Account> reg = new ArrayList<Account>();//Trusted obj within a trusted obj
public AccountRegistry() {}
public void addAccount(Account acc) {
this.reg.add(acc);
}}
@Untrusted
class Person {
	private String name;
	private Account acc;//Trusted obj within a untrusted obj.
	public Person(String name, int bal){
		this.name = name;
		this.acc = new Account(name,bal);	
	}	
	public Account getAccount(){
		return this.acc;
	}	
	public void transfer(Person receiver, int sum){
		receiver.getAccount().updateBalance(sum);
		this.acc.updateBalance(-sum);
}}

public static void main(String[] args) {
Person p1 = new Person("Alice",100);
Person p2 = new Person("Bob",25);
p1.transfer(p2,25);
AccountRegistry reg = new AccountRegistry();
reg.addAccount(p1.getAccount());	
}

\end{lstlisting}


\subsection{Partitioning language}
\label{sec:language}
%\begin{itemize}
%	\item Justify our approach: why code annotation instead of data partitioning (intuitive for the developer). 
%	\item Explain our annotation types
%	\item Use our example to illustrate
%\end{itemize}
When partitioning applications destined for enclaves, an important question which arises is how to specify what should be secured or not. 
Some recent works proposed annotation of sensitive data~\cite{glamdring}, others proposed annotation of sensitive routines~\cite{uranus,civet}. 
While these strategies work, we argue they are not always very intuitive for an application developer. 
Furthermore, they require complex and expensive data flow analysis to ensure sensitive data is not leaked. 

Instead, we propose a technique based on \textit{class annotations}.
Classes are a fundamental building block for object oriented applications, and it is very intuitive to reason about security along class boundaries.
Using annotations, developers can easily specify which class needs to be secured and which class needs not be secured.
\sys supports two principal annotations: \texttt{Trusted} and \texttt{Untrusted} which developers can use to specify secured and unsecured classes, respectively.
In Listing~\ref{lst:simple:1}, \texttt{Account} and \texttt{AccountRegistry} classes are annotated as trusted, while class \texttt{Person} is untrusted.

A \texttt{trusted} class will always be instantiated and manipulated inside the enclave.
This has two implications.
First, its member fields which are not instances of \texttt{untrusted} classes will be allocated on enclave's heap\vs{add example from Account}\vs{check if we mention earlier how enclave's heap and untrusted heap are maintained/init}.
Second, its methods are always executed inside the enclave.
Similarly for a class annotated as \texttt{Untrusted}, its objects will be allocated only on the untrusted heap, as well as all its member fields not instances of \texttt{Trusted} classes.
All its methods will be executed outside the enclave.
\sys maintains a single and the same copy/version of a \texttt{trusted} or an \texttt{untrusted} object in the two worlds leveraging \texttt{proxy} objects (see \S\ref{sec:byte-code-partitioning}).
In our programming model, some classes can be \texttt{Neutral} as they need not to be trusted or untrusted.
This is the case for utility classes such as \texttt{Arrays}, \texttt{Vector}, \texttt{String} or other similar application-specific classes (\ie added by the developer).
Such classes are not security sensitive and can be accessed in or out of the enclave without the used of proxies.
Contrary to \texttt{Trusted} and \texttt{Untrusted} classess, \texttt{neutral} classe instances can have several copies in both worlds, which can evolve independently. 
\texttt{Neutral} classes are not annotated.

%\vs{explicitely?}\py{inherent is the term..not explicitly..}
%\vs{personally i find 'Don't-care' not usefriendly as a term, with a dash and a \''. Could we use Ignored ?}
One may legitimately question the relevance of two annotations, thinking that the annotation \texttt{Trusted} is sufficiently expressive.
We could simply annotate trusted classes and consider unannotated classes as untrusted, to be instantiated out of the enclave.
This naive approach is not tractable because for an application to run inside the enclave, not only application specific trusted classes are needed, but also GraalVM runtime components and associated classes (\eg, the GC).
Considering a solution which keeps these classes out of the enclave is not tractable because of the number of ecall and ocall it will generate.
By allowing the developper to explicitely specify \texttt{Trusted} or \texttt{Untrusted} classes and keep the others \texttt{Neutral}, \sys is able to generate a native image for the enclave which will lead to fewer ecall/ocall.\vs{a reviewer might be believe that this trade-off will shown in the eval}

%\at{Peterson justifies why we need Untrusted annotation and Don't care. If explained below, give some few words which intuitively justify them, and ref the corresponding section. Some thing like this: One may wonder while xxxx.}

\smallskip\noindent\textbf{Assumptions}
We assume all annotated classes are fully encapsulated (\ie class fields are private). 
On the one hand, this prevents complex and expensive data flow analysis to prevent sensitive class fields from leaving the enclave \py{@Gael maybe you can expantiate here a little more :)}. 
On the other hand, it ensures that all class fields can only be accessed from outside classes via public methods \eg getters and setters exposed by the class. 
As such, it is easier to control access to these sensitive class fields by applying techniques such as transparent encryption/decryption at the level of these public methods. 
Encapsulation being one pillar of object orientation, we believe this assumption to be reasonable.

\subsection{Bytecode transformation}
\label{sec:byte-code-partitioning}
%\begin{itemize}
%	\item Partition at the byte code level. Explain why.
%	\item Proxy object creation
%	\item Parameter and return object management
%\end{itemize}
To better understand the purpose of this phase, we will begin by noting that the final partitioned application consists of two native images: a \textit{trusted} and an \textit{untrusted} image. 
The trusted image will not have any untrusted functionality, and the untrusted image will not have any trusted functionality. 
However, trusted objects (\ie instances of trusted classes) may call untrusted objects (\ie instances of untrusted classes) and vice versa. 
Hence, we need to have a way to access untrusted functionality from the trusted runtime and trusted functionality from the outside. 
To do this, we introduce the notion of \textit{proxy classes}. In the trusted runtime, we will have proxy classes for untrusted classes and in the untrusted runtime we will have untrusted proxy classes for the trusted classes. These proxies will serve as gateways to access the functionality (\ie methods) of the real class in the opposite runtime.The proxy classes expose the same methods as the original class, but do not perform any application specific functions themselves. Instead they perform enclave transitions at to access the real functionality in the opposite runtime. This design makes cross enclave object communication easier and helps maintaining the object oriented nature of the program as a whole after it is partitioned. We do bytecode transformations to \emph{create} these proxy classes and \emph{inject} code into existing classes to permit to do enclave transitions.
\sys uses Javassist~\cite{jassist}, a popular bytecode instrumentation framework, to achieve this phase.


For all trusted classes, \sys automatically introduces corresponding proxy classes, and for all untrusted classes, it introduces corresponding untrusted proxy classes. 
In \sys, the bytecode weaver is responsible for doing these bytecode transformations.
Notice that, we choose this approach of creating proxies for all annotated classes instead of only reachable classes during this phase because we know that the next phase performed by GraalVM will not include unreachable proxies in the generated native images (see Section\at{ref}).


Therefore, the byte code weaver in \sys works as follows, illustrated in listing\at{ref1,ref2,etc}.
\begin{lstlisting}[caption={Proxy class Account.}, label={lst:account-proxy}, basicstyle=\tiny]
public class Account {
private int hash;		
public Account(String name,int bal){
	byte[] buff = serialize(name);
	CCharPointer ptr = getPointer(buff);
	ecall_relay_Account(hash,ptr,bal);
}	
public void updateBalance(int val){
	ecall_relay_updateBalance(this.hash,val);
}}	
\end{lstlisting}

For the purposes of the trusted image, it creates proxy classes for untrusted classes by stripping the methods (\ie removing the method bodies) of the untrusted classes.
Listing\at{ref} shows the corresponding proxy class for the untrusted class \texttt{Person} in our illustrative example.
The bodies of the stripped methods are replaced with native routines which will perform Ocall transitions to the corresponding method in the untrusted runtime (lines \at{xx-xx} in listing\at{ref}).
Analogously, for untrusted image generation, the bytecode weaver creates proxy classes for trusted classes by stripping all methods of trusted classes, and replacing the method bodies with native methods which will perform Ecall transitions.
Listing\at{ref} shows the corresponding proxy class for the trusted class \texttt{xxx} in our illustrative example.
The proxy class fields are removed and an \texttt{id field} is added to each proxy class which stores the hash of the corresponding object (line \at{xxx} in listing\at{ref}). The result of these stripping operations is the removal from the trusted and untrusted runtime of all untrusted and trusted functionality respectively.
Only annotated classes are modified by the bytecode weaver \ie \texttt{neutral} classes are not changed.

In the following, we refer to all unstripped classes as \textit{concrete classes} and stripped classes as \textit{proxy classes}. We call the instances of these classes \textit{concrete objects} and \textit{proxy objects} respectively. If a concrete object in one runtime (trusted or untrusted) has a correspondence with a proxy object in the opposite runtime, we refer to that concrete object as a \textit{mirror object} (\ie the proxy's mirror copy).

%For the illustrative example, class \texttt{Person} will be made a proxy for trusted image generation, while classes \texttt{Account} and \texttt{AccountRegistry} will be made proxies for untrusted image generation.


\smallskip\noindent\textbf{Relay methods.}
For methods in one runtime (a native image) to be callable from the other runtime (another native image), these methods must be exported as \textit{entrypoints}. GraalVM Native Image provides an annotation (\texttt{@CEntryPoint}~\cite{centrypoint}) for specifying entrypoint methods which can be callable from C. These entrypoint methods must be static, may only have non-object parameters and return types \ie primitive types or Word types (including pointers)~\cite{graalSite}, and must specify the GraalVM isolate which will serve as execution context for the method. As a result of these restrictions, it is not feasible to export all methods of concrete classes as entrypoints directly, as this will mean changing their signatures. Our solution to this problem is to introduce static entrypoint methods which will act as wrappers for the invocations of the associated class or instance methods. We call these methods \textit{relay methods}. 

\sys bytecode weaver builds relay methods as follows.
For illustration, the relay method (\texttt{ecall\_relay\_Account}) will be woven into concrete class \texttt{Account} in the trusted runtime. The following code outlines the state of concrete class \texttt{Account} after bytecode weaving.
\begin{lstlisting}[caption={Concrete class \texttt{Account} after bytecode weaving.}, label={lst:account-relay}, basicstyle=\tiny]
public class Account {
private String owner;
private int balance;		
public Account(String name,int bal){...}
public void updateBalance(int val){...}

@CEntryPoint
public static void relay_Account(Isolate context,int hash,CCharPointer buff,int bal){
	String name = deserialize(buff);
	Account mirror = new Account(name,bal);
	mirrorProxyRegistry.add(hash,mirror);
}
@CEntryPoint
public static void relay_udpateBalance(Isolate context,int hash,int val){
	Account mirror = mirrorProxyRegistry.get(hash);
	mirror.updateBalance(val);
}}
\end{lstlisting}
For each method in a concrete class, including all constructors, the bytecode weaver adds an associated relay method to the class (line \at{xx} in listing xxx).
The native methods we add to the stripped methods of the proxy classes will perform enclave transitions to invoke the corresponding relay methods.

The parameters of a relay method comprise: the id of the calling proxy object (for non-static methods), all primitive parameters of the associated method, and pointers (~\ie \texttt{CCharPointer}~\cite{ccharpointer}) which represent the addresses of buffers obtained from the serialization of any object parameters which are instances of \texttt{neutral} classes (remember that the latter do not need proxies).
For proxy object parameters, the id of the corresponding proxy is passed as parameter and the corresponding mirror object will be used as the parameter once the real method is called in the opposite runtime. Similarly, for mirror object parameters, the id of the corresponding proxy is also sent, and the corresponding proxy object is used in the opposite runtime as parameter in the method.

About the serialized buffers, they are deserialized and the corresponding object parameter recreated in the body of the relay method.
For relay methods of constructors, we add code to instantiate the corresponding mirror object, and code to add the mirror object strong reference - proxy id pair to a global registry, which we call the \textit{mirror-proxy registry}. For instance methods, we add code to look up the corresponding mirror object in the registry, and then invoke the instance method on that mirror object with its corresponding parameters. Neutral object return types from the untrusted runtime are also serialized and copied across the enclave boundary. Both the trusted and untrusted runtimes have a mirror-proxy registry.


We complete the transformation of the other classes of our illustrative example as follows.
For proxy class \texttt{Person}, we will have Ocalls instead to the relay methods.
For proxy class \texttt{AccountRegistry}, we have a proxy \texttt{Account} as parameter in the \texttt{addAccount} method.
Only its id will be passed to the opposite runtime.
The resulting proxy method will be as follows:

\begin{lstlisting}[label={lst:simple}, basicstyle=\tiny]
public void addAccount(Account acc){
ecall_relay_addAccount(acc.getHash());
}
\end{lstlisting}

The corresponding relay method in concrete class\\ \texttt{AccountRegistry} will be as follows:
\begin{lstlisting}[label={lst:simple}, basicstyle=\tiny]
@CEntryPoint
public static void relay_addAccount(Isolate context,int hash){
Account mirror = mirrorProxyRegistry.get(hash);
this.addAccount(mirror);
}
\end{lstlisting}

\smallskip\noindent\textbf{Native transition methods.}
The native transition methods (\eg \texttt{ecall\_addAccount }\etc) are C routines which perform enclave transitions to the opposite runtime. At the time of bytecode transformation, the definitions of the native transition methods are absent and only their signatures are provided. Their definitions will be generated by the native image generator (see the next section). 



\subsection{Native image partitioning}
\label{sec:native-image-partitioning}
%\begin{itemize}
%	\item How we decide which runtime class should be integrated into the enclave native image
%	\item Entry classes
%	\item Isolates?
%	\item sgx wrappers
%\end{itemize}
The GraalVM native image generator is responsible for building native images. It takes as input compiled application classes (bytecode), and all their associated external libraries, including the JDK; we note the set of external libraries as \texttt{L}. The native image generator then performs points-to analysis~\cite{nativeImgs} (\ie static analysis) to find the reachable program elements (\ie classes, methods and fields). Only reachable methods are then ahead-of-time compiled into the final native image. For an SGX-based environment, this is particularly useful as it permits to exclude any redundant application logic from the enclave. The resulting image includes runtime components for garbage collection (memory management), thread scheduling, deoptimization \etc. Substrate VM (SVM) is the collective name for these components in GraalVM. 

\smallskip\noindent\textbf{Static analysis for trusted and untrusted image generation.}
The bytecode weaving process produced two sets of class files: the first set (\texttt{T}) comprises modified trusted classes and untrusted proxy classes, while the second set (\texttt{U}) comprises modified untrusted classes and secure proxy classes. The set of 
unannotated/\texttt{neutral} classes (\texttt{N}) were not changed by the bytecode weaver. These 3 sets of classes are used by GraalVM to generate two native images which represent the partitioned application.

In \sys, the native image generator uses set ($T\cup N\cup L$) as input for \textit{trusted image} generation and the set ($U\cup N\cup L$) as input for \textit{untrusted image} generation. To determine reachable program elements (\ie classes, methods and fields) the native image generator leverages a static analysis technique known as points-to analysis~\cite{nativeImgs,balatsouras}. Points-to analysis starts with all entrypoints and iteratively processes all transitively reachable methods~\cite{nativeImgs}. For the sake of brevity, we do not include all the steps performed during points-to analysis in GraalVM Native Image, as this is extensively handled by prior work~\cite{nativeImgs}. For the trusted image, all the relay methods of trusted classes will serve as entrypoints (recall the \texttt{@CEntryPoint} annotation \eg listing~\ref{lst:account-relay}). For the untrusted image, the main entrypoint (\ie Java application main) and the relay methods of untrusted classes will serve as entrypoints. Conceptually, we can include the main entrypoint in either the trusted or untrusted image. However we chose to add it in the untrusted image because: (1) it prevents an Ecall transition to invoke the main method, and Ocall transitions to create garbage collection helper threads (see \S\ref{sec:gc}) once in the main method, (2) it is in accordance with Intel SGX's programming convention, as all SGX applications begin in the untrusted runtime.

Figure \ref{fig:call-graphs} illustrates a condensed reachability analysis done two entrypoint methods (\texttt{relay\_Account} and \texttt{main}) to determine their reachable methods. A similar thing is done for all other entrypoints.

\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.25]{fig/call_graphs}	
	\caption{For the trusted image, the relay methods in the trusted classes make other trusted class methods reachable, as well as methods from neutral classes (\eg \texttt{serialize}, \texttt{registry.add} \etc). Similarly, for the untrusted image, the main entrypoint makes the \texttt{Person} class methods reachable, as well as methods from proxy classes \texttt{Account} and \texttt{AccountRegistry}.}
	\label{fig:call-graphs}
\end{figure}

After static analysis is complete, the trusted image will not contain untrusted methods/functionality. It will have proxies to those if some untrusted proxy class methods were reachable. Similarly, the untrusted image will not contain trusted methods, only proxies to those if some proxy class methods were reachable. 

So for the \texttt{main} method in our illustrative example~\ref{lst:main}, at runtime during object creation for \texttt{Person} $p1$ and $p2$, their constructors will instantiate a proxy object of the \texttt{proxy Account class}. The String parameters \texttt{"Alice"} and \texttt{"Bob"} will be serialized and an Ecall transition will be made to create a corresponding \texttt{mirror Account object} in the enclave. Similarly, when \texttt{p1.transfer(p2,25)} is called, the corresponding \texttt{proxy Account objects} will perform enclave transitions to update the balances in the enclave. In the same way, the call to \texttt{proxy AccountRegistry} constructor performs a transition to create a mirror object in the enclave corresponding to proxy object \texttt{reg}. The latter performs a transition too when \texttt{addAccount} is called.


%We modified GraalVM's default native image builder to generate these two images for each application to be partitioned. 
By default, GraalVM's image generator compiles all reachable methods and links the latter with GraalVM's native libraries to produce an executable or a shared object file. We modified the image generator to bypass the linking phase that produces executables or shared objects, so as to produce relocatable object files (.o) which can be linked to other libraries to build the final SGX application. The resulting images for the trusted and untrusted parts are \texttt{trusted.o} and \texttt{untrusted.o} respectively. These will be dispatched to the SGX module and used to build the final SGX application.


%NB: speculative optimization can be done in a program based on profiling data collected during program execution e.g type specializations for interfaces. If the program invalidates these assumptions at runtime, e.g when a second class implementing the said interface is loaded, deoptimizations will need to be done at the level of the VM 

\smallskip\noindent\textbf{SGX code generator.}
During bytecode weaving, native transition routines (Ecalls and Ocalls) were added to proxy classes. We extended GraalVM's native image builder with a class to generate C code definitions for the corresponding Ecalls (added in trusted proxy classes) or Ocalls (added in untrusted proxy classes), as well as their corresponding header files. As an example, listing~\ref{lst:ecall-addAccount} shows the generated C code for the \texttt{ecall\_relay\_addAccount} method.

\begin{lstlisting}[label={lst:ecall-addAccount}]

void ecall_relay_addAccount(int hash){
//this will return the enclave isolate
Isolate iso = getIsolate();
relay_addAccount(iso,hash);
}
\end{lstlisting}

The code generator also creates associated EDL files which will be used by the Edger8r tool in the Intel SGX SDK to build bridge routines which will help in marshalling data across the enclave boundary. The generated files are dispatched to the SGX module.

\subsection{SGX application creation}
\label{sec:sgx-app-creation}
This is the final stage in the \sys workflow. The \textit{SGX module} is the component responsible for building the final SGX application based on the generated native images. This module builds SGX applications following the standard Intel SGX SDK application design which requires the application to be divided into trusted and untrusted components. %The trusted components and compiled together to produce the final enclave shared object which is loaded in secure memory at runtime.

Because SGX enclaves operate only in user mode, they cannot issue system calls and standard OS abstractions (e.g., file systems, network), which are ubiquitous in real world applications. The solution to this problem is to relay these unsupported calls to the untrusted runtime, which does not have the same limitations. In contrast to systems which introduce a LibOS into the enclave, we leverage an approach which involves redefining unsupported libc routines as wrappers for ocalls. These redefined libc routines in the enclave constitute the \textit{shim library}. The latter intercepts calls to libc routines and relays them to the untrusted runtime. A \textit{shim helper library} in the untrusted runtime then invokes the real libc routines. This by design reduces the TCB when compared to LibOS-based systems.


The SGX module compiles all generated Ecalls and statically links the latter with the trusted image (\texttt{trusted.o}), the shim library, and native libraries from GraalVM to produce the final enclave shared library which corresponds to the trusted component of the SGX application. Similarly, the generated Ocalls are also compiled and linked with the untrusted image (\texttt{untrusted.o}) and GraalVM native libraries to produce the final untrusted component. In accordance with Intel SGX's application model, we compile the main entrypoint of partitioned applications in the untrusted component. The resulting trusted and untrusted components comprise the final SGX application. 

%Following our illustrative example, consider the following main routine executing in the untrusted runtime:


%During object creating for \texttt{Person} $p1$ and $p2$ their constructors will instantiate a proxy object of the \texttt{proxy Account class}. The String parameters \texttt{"Alice"} and \texttt{"Bob"} will be serialized and an Ecall transition will be made to create a corresponding \texttt{mirror Account object} in the enclave. Similarly, when \texttt{p1.transfer(p2,25)} is called, the corresponding \texttt{proxy Account objects} will perform enclave transitions to update the balances in the enclave. In the same way, the call to \texttt{proxy AccountRegistry} constructor performs a transition to create a mirror object in the enclave corresponding to proxy object \texttt{reg}. The latter performs a transition too when \texttt{addAccount} is called.

\subsection{Garbage collection}
\label{sec:gc}
%\begin{itemize}
%	\item Two GC
%	\item Describe the GC of each world
%\end{itemize}

Following our partitioned application design, untrusted code objects can have trusted counterparts and vice versa. This presents a challenge at the level of garbage collection because we must ensure synchronized destruction of objects across the trusted and untrusted heaps. More specifically, we need to synchronize GC of proxy and mirror objects; \eg the mirror of proxy object \texttt{reg} should not be destroyed before \texttt{reg}.

To address this problem, we implemented an application level GC helper. When a proxy object is created, we store a weak reference to it in a global list, as well as its id. The GC helper thread periodically scans this list for null weak references. Once such a null weak reference is found, it means the corresponding proxy object has been garbage collected, and thus we can remove the mirror object from the mirror-proxy registry in the opposite runtime. Both the trusted and untrusted runtimes maintain independent lists of proxy weak references for the associated runtime, and two GC helper threads are spawned in the application: one to scan the trusted list in the enclave, and the other to scan the untrusted list. Algorithm \ref{alg:gc-helper} outlines the work of the GC helper thread. 


\begin{algorithm}[th]
	\caption{GC helper thread.}
	\label{alg:gc-helper}
	\begin{algorithmic}[1]
		\State $\mathit{proxyWeakRefs} \gets \{\mathit{list~of~proxy~obj~weak~refs}\}$
		\While {!stopped}
		\State $wait(TIME)$
		\ForAll{$ref\in\mathit{proxyWeakRefs}$}
		\If{$ref = null$}
		\State $\mathit{proxyId} \gets \mathit{getProxyId()}$
		\If{$inEnclave$}
		\State $\mathit{ocall\_removeMirror(proxyId)}$ 					
		\Else
		\State $\mathit{ecall\_removeMirror(proxyId)}$ 
		\EndIf
		\State $\mathit{proxyWeakRefs}\gets \mathit{proxyWeakRefs}\setminus \mathit{ref}$
		\EndIf
		\EndFor
		\EndWhile
	\end{algorithmic}
\end{algorithm}



The \texttt{removeMirror} ocalls or ecalls perform an enclave transition which removes the mirror object - proxy id pair from the corresponding mirror-proxy registry. This automatically makes the mirror object eligible for GC if it is not strongly referenced somewhere else in the program.


\subsection{Running unpartitioned native images in \sys}
Inspite of the benefits of partitioning an enclave application, situations may arise where it is much easier for the application developer to run the entire application as a native image in the enclave. This could happen when the majority of classes potentially deal with sensitive information and no classes qualify as untrusted. For this, we offer the possibility to run the unpartitioned application with \sys. Here no annotations are required and hence no bytecode modifications are done. The original application is built into a single native image which is linked entirely to the final enclave object. Running the entire native image in an enclave increases the TCB but we argue here that the TCB increase is small relative to the same application running on a full-blown JVM in an enclave. Furthermore, the increased heap size due to the entire JVM in the enclave could strain the EPC leading to performance degradations in the application.









==> bib-header.tex <==
% Journals

% First the Full Name is given, then the abbreviation used in the AMS Math
% Reviews, with an indication if it could not be found there.
% Note the 2nd overwrites the 1st, so swap them if you want the full name.

 %{AMS}
 @String{AMSTrans = "American Mathematical Society Translations" }
 @String{AMSTrans = "Amer. Math. Soc. Transl." }
 @String{BullAMS = "Bulletin of the American Mathematical Society" }
 @String{BullAMS = "Bull. Amer. Math. Soc." }
 @String{ProcAMS = "Proceedings of the American Mathematical Society" }
 @String{ProcAMS = "Proc. Amer. Math. Soc." }
 @String{TransAMS = "Transactions of the American Mathematical Society" }
 @String{TransAMS = "Trans. Amer. Math. Soc." }

 %ACM
 @String{CACM = "Communications of the {ACM}" }
 @String{CACM = "Commun. {ACM}" }
 @String{CompServ = "Comput. Surveys" }
 @String{JACM = "J. ACM" }
 @String{ACMMathSoft = "{ACM} Transactions on Mathematical Software" }
 @String{ACMMathSoft = "{ACM} Trans. Math. Software" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newsletter" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newslett." }

 @String{AmerSocio = "American Journal of Sociology" }
 @String{AmerStatAssoc = "Journal of the American Statistical Association" }
 @String{AmerStatAssoc = "J. Amer. Statist. Assoc." }
 @String{ApplMathComp = "Applied Mathematics and Computation" }
 @String{ApplMathComp = "Appl. Math. Comput." }
 @String{AmerMathMonthly = "American Mathematical Monthly" }
 @String{AmerMathMonthly = "Amer. Math. Monthly" }
 @String{BIT = "{BIT}" }
 @String{BritStatPsych = "British Journal of Mathematical and Statistical
          Psychology" }
 @String{BritStatPsych = "Brit. J. Math. Statist. Psych." }
 @String{CanMathBull = "Canadian Mathematical Bulletin" }
 @String{CanMathBull = "Canad. Math. Bull." }
 @String{CompApplMath = "Journal of Computational and Applied Mathematics" }
 @String{CompApplMath = "J. Comput. Appl. Math." }
 @String{CompPhys = "Journal of Computational Physics" }
 @String{CompPhys = "J. Comput. Phys." }
 @String{CompStruct = "Computers and Structures" }
 @String{CompStruct = "Comput. \& Structures" }
 @String{CompJour = "The Computer Journal" }
 @String{CompJour = "Comput. J." }
 @String{CompSysSci = "Journal of Computer and System Sciences" }
 @String{CompSysSci = "J. Comput. System Sci." }
 @String{Computing = "Computing" }
 @String{ContempMath = "Contemporary Mathematics" }
 @String{ContempMath = "Contemp. Math." }
 @String{Crelle = "Crelle's Journal" }
 @String{GiornaleMath = "Giornale di Mathematiche" }
 @String{GiornaleMath = "Giorn. Mat." } % didn't find in AMS MR., ibid.

 %IEEE
 @String{Computer = "{IEEE} Computer" }
 @String{IEEETransComp = "{IEEE} Transactions on Computers" }
 @String{IEEETransComp = "{IEEE} Trans. Comput." }
 @String{IEEETransAC = "{IEEE} Transactions on Automatic Control" }
 @String{IEEETransAC = "{IEEE} Trans. Automat. Control" }
 @String{IEEESpec = "{IEEE} Spectrum" } % didn't find in AMS MR
 @String{ProcIEEE = "Proceedings of the {IEEE}" }
 @String{ProcIEEE = "Proc. {IEEE}" } % didn't find in AMS MR
 @String{IEEETransAeroElec = "{IEEE} Transactions on Aerospace and Electronic
     Systems" }
 @String{IEEETransAeroElec = "{IEEE} Trans. Aerospace Electron. Systems" }

 @String{IMANumerAna = "{IMA} Journal of Numerical Analysis" }
 @String{IMANumerAna = "{IMA} J. Numer. Anal." }
 @String{InfProcLet = "Information Processing Letters" }
 @String{InfProcLet = "Inform. Process. Lett." }
 @String{InstMathApp = "Journal of the Institute of Mathematics and
     its Applications" }
 @String{InstMathApp = "J. Inst. Math. Appl." }
 @String{IntControl = "International Journal of Control" }
 @String{IntControl = "Internat. J. Control" }
 @String{IntNumerEng = "International Journal for Numerical Methods in
     Engineering" }
 @String{IntNumerEng = "Internat. J. Numer. Methods Engrg." }
 @String{IntSuper = "International Journal of Supercomputing Applications" }
 @String{IntSuper = "Internat. J. Supercomputing Applic." } % didn't find
%% in AMS MR
 @String{Kibernetika = "Kibernetika" }
 @String{JResNatBurStand = "Journal of Research of the National Bureau
     of Standards" }
 @String{JResNatBurStand = "J. Res. Nat. Bur. Standards" }
 @String{LinAlgApp = "Linear Algebra and its Applications" }
 @String{LinAlgApp = "Linear Algebra Appl." }
 @String{MathAnaAppl = "Journal of Mathematical Analysis and Applications" }
 @String{MathAnaAppl = "J. Math. Anal. Appl." }
 @String{MathAnnalen = "Mathematische Annalen" }
 @String{MathAnnalen = "Math. Ann." }
 @String{MathPhys = "Journal of Mathematical Physics" }
 @String{MathPhys = "J. Math. Phys." }
 @String{MathComp = "Mathematics of Computation" }
 @String{MathComp = "Math. Comp." }
 @String{MathScand = "Mathematica Scandinavica" }
 @String{MathScand = "Math. Scand." }
 @String{TablesAidsComp = "Mathematical Tables and Other Aids to Computation" }
 @String{TablesAidsComp = "Math. Tables Aids Comput." }
 @String{NumerMath = "Numerische Mathematik" }
 @String{NumerMath = "Numer. Math." }
 @String{PacificMath = "Pacific Journal of Mathematics" }
 @String{PacificMath = "Pacific J. Math." }
 @String{ParDistComp = "Journal of Parallel and Distributed Computing" }
 @String{ParDistComp = "J. Parallel and Distrib. Comput." } % didn't find
%% in AMS MR
 @String{ParComputing = "Parallel Computing" }
 @String{ParComputing = "Parallel Comput." }
 @String{PhilMag = "Philosophical Magazine" }
 @String{PhilMag = "Philos. Mag." }
 @String{ProcNAS = "Proceedings of the National Academy of Sciences
                    of the USA" }
 @String{ProcNAS = "Proc. Nat. Acad. Sci. U. S. A." }
 @String{Psychometrika = "Psychometrika" }
 @String{QuartMath = "Quarterly Journal of Mathematics, Oxford, Series (2)" }
 @String{QuartMath = "Quart. J. Math. Oxford Ser. (2)" }
 @String{QuartApplMath = "Quarterly of Applied Mathematics" }
 @String{QuartApplMath = "Quart. Appl. Math." }
 @String{RevueInstStat = "Review of the International Statisical Institute" }
 @String{RevueInstStat = "Rev. Inst. Internat. Statist." }

 %SIAM
 @String{JSIAM = "Journal of the Society for Industrial and Applied
     Mathematics" }
 @String{JSIAM = "J. Soc. Indust. Appl. Math." }
 @String{JSIAMB = "Journal of the Society for Industrial and Applied
     Mathematics, Series B, Numerical Analysis" }
 @String{JSIAMB = "J. Soc. Indust. Appl. Math. Ser. B Numer. Anal." }
 @String{SIAMAlgMeth = "{SIAM} Journal on Algebraic and Discrete Methods" }
 @String{SIAMAlgMeth = "{SIAM} J. Algebraic Discrete Methods" }
 @String{SIAMAppMath = "{SIAM} Journal on Applied Mathematics" }
 @String{SIAMAppMath = "{SIAM} J. Appl. Math." }
 @String{SIAMComp = "{SIAM} Journal on Computing" }
 @String{SIAMComp = "{SIAM} J. Comput." }
 @String{SIAMMatrix = "{SIAM} Journal on Matrix Analysis and Applications" }
 @String{SIAMMatrix = "{SIAM} J. Matrix Anal. Appl." }
 @String{SIAMNumAnal = "{SIAM} Journal on Numerical Analysis" }
 @String{SIAMNumAnal = "{SIAM} J. Numer. Anal." }
 @String{SIAMReview = "{SIAM} Review" }
 @String{SIAMReview = "{SIAM} Rev." }
 @String{SIAMSciStat = "{SIAM} Journal on Scientific and Statistical
     Computing" }
 @String{SIAMSciStat = "{SIAM} J. Sci. Statist. Comput." }

 @String{SoftPracExp = "Software Practice and Experience" }
 @String{SoftPracExp = "Software Prac. Experience" } % didn't find in AMS MR
 @String{StatScience = "Statistical Science" }
 @String{StatScience = "Statist. Sci." }
 @String{Techno = "Technometrics" }
 @String{USSRCompMathPhys = "{USSR} Computational Mathematics and Mathematical
     Physics" }
 @String{USSRCompMathPhys = "{U. S. S. R.} Comput. Math. and Math. Phys." }
 @String{VLSICompSys = "Journal of {VLSI} and Computer Systems" }
 @String{VLSICompSys = "J. {VLSI} Comput. Syst." }
 @String{ZAngewMathMech = "Zeitschrift fur Angewandte Mathematik und
     Mechanik" }
 @String{ZAngewMathMech = "Z. Angew. Math. Mech." }
 @String{ZAngewMathPhys = "Zeitschrift fur Angewandte Mathematik und Physik" }
 @String{ZAngewMathPhys = "Z. Angew. Math. Phys." }

% Publishers % ================================================= |

 @String{Academic = "Academic Press" }
 @String{ACMPress = "{ACM} Press" }
 @String{AdamHilger = "Adam Hilger" }
 @String{AddisonWesley = "Addison-Wesley" }
 @String{AllynBacon = "Allyn and Bacon" }
 @String{AMS = "American Mathematical Society" }
 @String{Birkhauser = "Birkha{\"u}ser" }
 @String{CambridgePress = "Cambridge University Press" }
 @String{Chelsea = "Chelsea" }
 @String{ClaredonPress = "Claredon Press" }
 @String{DoverPub = "Dover Publications" }
 @String{Eyolles = "Eyolles" }
 @String{HoltRinehartWinston = "Holt, Rinehart and Winston" }
 @String{Interscience = "Interscience" }
 @String{JohnsHopkinsPress = "The Johns Hopkins University Press" }
 @String{JohnWileySons = "John Wiley and Sons" }
 @String{Macmillan = "Macmillan" }
 @String{MathWorks = "The Math Works Inc." }
 @String{McGrawHill = "McGraw-Hill" }
 @String{NatBurStd = "National Bureau of Standards" }
 @String{NorthHolland = "North-Holland" }
 @String{OxfordPress = "Oxford University Press" }  %address Oxford or London?
 @String{PergamonPress = "Pergamon Press" }
 @String{PlenumPress = "Plenum Press" }
 @String{PrenticeHall = "Prentice-Hall" }
 @String{SIAMPub = "{SIAM} Publications" }
 @String{Springer = "Springer-Verlag" }
 @String{TexasPress = "University of Texas Press" }
 @String{VanNostrand = "Van Nostrand" }
 @String{WHFreeman = "W. H. Freeman and Co." }

==> implementation.tex <==
%!TEX root = main.tex

%\section{Implementation}
%\label{sec:implementation}
%We implement \sys based on GraalVM CE v21.0.0 for Java 8. GraalVM and the bytecode weaver are implemented in Java. Our modifications in GraalVM amount to $\sim 1400$ lines of code (LOC). The bytecode weaver is based on Javassist v3.26 and is $\sim2100$ LOC. The SGX module is based on SGX SDK and SGX driver v2.11, is implemented in C/C++, and is $\sim 46k$ LOC.




==> journals.tex <==
% Journals

% First the Full Name is given, then the abbreviation used in the AMS Math
% Reviews, with an indication if it could not be found there.
% Note the 2nd overwrites the 1st, so swap them if you want the full name.

 %{AMS}
 @String{AMSTrans = "American Mathematical Society Translations" }
 @String{AMSTrans = "Amer. Math. Soc. Transl." }
 @String{BullAMS = "Bulletin of the American Mathematical Society" }
 @String{BullAMS = "Bull. Amer. Math. Soc." }
 @String{ProcAMS = "Proceedings of the American Mathematical Society" }
 @String{ProcAMS = "Proc. Amer. Math. Soc." }
 @String{TransAMS = "Transactions of the American Mathematical Society" }
 @String{TransAMS = "Trans. Amer. Math. Soc." }

 %ACM
 @String{CACM = "Communications of the {ACM}" }
 @String{CACM = "Commun. {ACM}" }
 @String{CompServ = "Comput. Surveys" }
 @String{JACM = "J. ACM" }
 @String{ACMMathSoft = "{ACM} Transactions on Mathematical Software" }
 @String{ACMMathSoft = "{ACM} Trans. Math. Software" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newsletter" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newslett." }

 @String{AmerSocio = "American Journal of Sociology" }
 @String{AmerStatAssoc = "Journal of the American Statistical Association" }
 @String{AmerStatAssoc = "J. Amer. Statist. Assoc." }
 @String{ApplMathComp = "Applied Mathematics and Computation" }
 @String{ApplMathComp = "Appl. Math. Comput." }
 @String{AmerMathMonthly = "American Mathematical Monthly" }
 @String{AmerMathMonthly = "Amer. Math. Monthly" }
 @String{BIT = "{BIT}" }
 @String{BritStatPsych = "British Journal of Mathematical and Statistical
          Psychology" }
 @String{BritStatPsych = "Brit. J. Math. Statist. Psych." }
 @String{CanMathBull = "Canadian Mathematical Bulletin" }
 @String{CanMathBull = "Canad. Math. Bull." }
 @String{CompApplMath = "Journal of Computational and Applied Mathematics" }
 @String{CompApplMath = "J. Comput. Appl. Math." }
 @String{CompPhys = "Journal of Computational Physics" }
 @String{CompPhys = "J. Comput. Phys." }
 @String{CompStruct = "Computers and Structures" }
 @String{CompStruct = "Comput. \& Structures" }
 @String{CompJour = "The Computer Journal" }
 @String{CompJour = "Comput. J." }
 @String{CompSysSci = "Journal of Computer and System Sciences" }
 @String{CompSysSci = "J. Comput. System Sci." }
 @String{Computing = "Computing" }
 @String{ContempMath = "Contemporary Mathematics" }
 @String{ContempMath = "Contemp. Math." }
 @String{Crelle = "Crelle's Journal" }
 @String{GiornaleMath = "Giornale di Mathematiche" }
 @String{GiornaleMath = "Giorn. Mat." } % didn't find in AMS MR., ibid.

 %IEEE
 @String{Computer = "{IEEE} Computer" }
 @String{IEEETransComp = "{IEEE} Transactions on Computers" }
 @String{IEEETransComp = "{IEEE} Trans. Comput." }
 @String{IEEETransAC = "{IEEE} Transactions on Automatic Control" }
 @String{IEEETransAC = "{IEEE} Trans. Automat. Control" }
 @String{IEEESpec = "{IEEE} Spectrum" } % didn't find in AMS MR
 @String{ProcIEEE = "Proceedings of the {IEEE}" }
 @String{ProcIEEE = "Proc. {IEEE}" } % didn't find in AMS MR
 @String{IEEETransAeroElec = "{IEEE} Transactions on Aerospace and Electronic
     Systems" }
 @String{IEEETransAeroElec = "{IEEE} Trans. Aerospace Electron. Systems" }

 @String{IMANumerAna = "{IMA} Journal of Numerical Analysis" }
 @String{IMANumerAna = "{IMA} J. Numer. Anal." }
 @String{InfProcLet = "Information Processing Letters" }
 @String{InfProcLet = "Inform. Process. Lett." }
 @String{InstMathApp = "Journal of the Institute of Mathematics and
     its Applications" }
 @String{InstMathApp = "J. Inst. Math. Appl." }
 @String{IntControl = "International Journal of Control" }
 @String{IntControl = "Internat. J. Control" }
 @String{IntNumerEng = "International Journal for Numerical Methods in
     Engineering" }
 @String{IntNumerEng = "Internat. J. Numer. Methods Engrg." }
 @String{IntSuper = "International Journal of Supercomputing Applications" }
 @String{IntSuper = "Internat. J. Supercomputing Applic." } % didn't find
%% in AMS MR
 @String{Kibernetika = "Kibernetika" }
 @String{JResNatBurStand = "Journal of Research of the National Bureau
     of Standards" }
 @String{JResNatBurStand = "J. Res. Nat. Bur. Standards" }
 @String{LinAlgApp = "Linear Algebra and its Applications" }
 @String{LinAlgApp = "Linear Algebra Appl." }
 @String{MathAnaAppl = "Journal of Mathematical Analysis and Applications" }
 @String{MathAnaAppl = "J. Math. Anal. Appl." }
 @String{MathAnnalen = "Mathematische Annalen" }
 @String{MathAnnalen = "Math. Ann." }
 @String{MathPhys = "Journal of Mathematical Physics" }
 @String{MathPhys = "J. Math. Phys." }
 @String{MathComp = "Mathematics of Computation" }
 @String{MathComp = "Math. Comp." }
 @String{MathScand = "Mathematica Scandinavica" }
 @String{MathScand = "Math. Scand." }
 @String{TablesAidsComp = "Mathematical Tables and Other Aids to Computation" }
 @String{TablesAidsComp = "Math. Tables Aids Comput." }
 @String{NumerMath = "Numerische Mathematik" }
 @String{NumerMath = "Numer. Math." }
 @String{PacificMath = "Pacific Journal of Mathematics" }
 @String{PacificMath = "Pacific J. Math." }
 @String{ParDistComp = "Journal of Parallel and Distributed Computing" }
 @String{ParDistComp = "J. Parallel and Distrib. Comput." } % didn't find
%% in AMS MR
 @String{ParComputing = "Parallel Computing" }
 @String{ParComputing = "Parallel Comput." }
 @String{PhilMag = "Philosophical Magazine" }
 @String{PhilMag = "Philos. Mag." }
 @String{ProcNAS = "Proceedings of the National Academy of Sciences
                    of the USA" }
 @String{ProcNAS = "Proc. Nat. Acad. Sci. U. S. A." }
 @String{Psychometrika = "Psychometrika" }
 @String{QuartMath = "Quarterly Journal of Mathematics, Oxford, Series (2)" }
 @String{QuartMath = "Quart. J. Math. Oxford Ser. (2)" }
 @String{QuartApplMath = "Quarterly of Applied Mathematics" }
 @String{QuartApplMath = "Quart. Appl. Math." }
 @String{RevueInstStat = "Review of the International Statisical Institute" }
 @String{RevueInstStat = "Rev. Inst. Internat. Statist." }

 %SIAM
 @String{JSIAM = "Journal of the Society for Industrial and Applied
     Mathematics" }
 @String{JSIAM = "J. Soc. Indust. Appl. Math." }
 @String{JSIAMB = "Journal of the Society for Industrial and Applied
     Mathematics, Series B, Numerical Analysis" }
 @String{JSIAMB = "J. Soc. Indust. Appl. Math. Ser. B Numer. Anal." }
 @String{SIAMAlgMeth = "{SIAM} Journal on Algebraic and Discrete Methods" }
 @String{SIAMAlgMeth = "{SIAM} J. Algebraic Discrete Methods" }
 @String{SIAMAppMath = "{SIAM} Journal on Applied Mathematics" }
 @String{SIAMAppMath = "{SIAM} J. Appl. Math." }
 @String{SIAMComp = "{SIAM} Journal on Computing" }
 @String{SIAMComp = "{SIAM} J. Comput." }
 @String{SIAMMatrix = "{SIAM} Journal on Matrix Analysis and Applications" }
 @String{SIAMMatrix = "{SIAM} J. Matrix Anal. Appl." }
 @String{SIAMNumAnal = "{SIAM} Journal on Numerical Analysis" }
 @String{SIAMNumAnal = "{SIAM} J. Numer. Anal." }
 @String{SIAMReview = "{SIAM} Review" }
 @String{SIAMReview = "{SIAM} Rev." }
 @String{SIAMSciStat = "{SIAM} Journal on Scientific and Statistical
     Computing" }
 @String{SIAMSciStat = "{SIAM} J. Sci. Statist. Comput." }

 @String{SoftPracExp = "Software Practice and Experience" }
 @String{SoftPracExp = "Software Prac. Experience" } % didn't find in AMS MR
 @String{StatScience = "Statistical Science" }
 @String{StatScience = "Statist. Sci." }
 @String{Techno = "Technometrics" }
 @String{USSRCompMathPhys = "{USSR} Computational Mathematics and Mathematical
     Physics" }
 @String{USSRCompMathPhys = "{U. S. S. R.} Comput. Math. and Math. Phys." }
 @String{VLSICompSys = "Journal of {VLSI} and Computer Systems" }
 @String{VLSICompSys = "J. {VLSI} Comput. Syst." }
 @String{ZAngewMathMech = "Zeitschrift fur Angewandte Mathematik und
     Mechanik" }
 @String{ZAngewMathMech = "Z. Angew. Math. Mech." }
 @String{ZAngewMathPhys = "Zeitschrift fur Angewandte Mathematik und Physik" }
 @String{ZAngewMathPhys = "Z. Angew. Math. Phys." }

% Publishers % ================================================= |

 @String{Academic = "Academic Press" }
 @String{ACMPress = "{ACM} Press" }
 @String{AdamHilger = "Adam Hilger" }
 @String{AddisonWesley = "Addison-Wesley" }
 @String{AllynBacon = "Allyn and Bacon" }
 @String{AMS = "American Mathematical Society" }
 @String{Birkhauser = "Birkha{\"u}ser" }
 @String{CambridgePress = "Cambridge University Press" }
 @String{Chelsea = "Chelsea" }
 @String{ClaredonPress = "Claredon Press" }
 @String{DoverPub = "Dover Publications" }
 @String{Eyolles = "Eyolles" }
 @String{HoltRinehartWinston = "Holt, Rinehart and Winston" }
 @String{Interscience = "Interscience" }
 @String{JohnsHopkinsPress = "The Johns Hopkins University Press" }
 @String{JohnWileySons = "John Wiley and Sons" }
 @String{Macmillan = "Macmillan" }
 @String{MathWorks = "The Math Works Inc." }
 @String{McGrawHill = "McGraw-Hill" }
 @String{NatBurStd = "National Bureau of Standards" }
 @String{NorthHolland = "North-Holland" }
 @String{OxfordPress = "Oxford University Press" }  %address Oxford or London?
 @String{PergamonPress = "Pergamon Press" }
 @String{PlenumPress = "Plenum Press" }
 @String{PrenticeHall = "Prentice-Hall" }
 @String{SIAMPub = "{SIAM} Publications" }
 @String{Springer = "Springer-Verlag" }
 @String{TexasPress = "University of Texas Press" }
 @String{VanNostrand = "Van Nostrand" }
 @String{WHFreeman = "W. H. Freeman and Co." }

==> limitations.tex <==
\section{Limitations and future work}
\label{sec:limitations}

\smallskip\noindent\textbf{Remote method invocations.}
Our results on proxy method creation and remote method invocations suggest that they introduce additional overhead when compared to regular object creation and method invocations.
This overhead should not greatly affect the performance of applications that do a small number of proxy creation and RMIs.
However the overhead could become more important when this number increases.
In this light, we plan to improve our RMI system by doing transition-less cross-enclave calls for expensive RMIs.
Prior work~\cite{switchless} has provided mechanisms to perform cross enclave calls without leaving the enclave.


\smallskip\noindent\textbf{Isolate design.}
All threads in a \graal native image execute within the context of a given \graal isolate.
Our present design creates default isolates for both the trusted and untrusted native images and communication between proxy and mirror object pairs only make sense for these two default isolates.
We will need to extend our proxy-mirror system to permit creation and interaction of proxy-mirror object pairs across multiple isolates in both the trusted and untrusted runtimes.


==> motivation.tex <==
%!TEX root = main.tex
%\vspace{-10pt}
\subsection{Motivation}
\label{sec:motivation}
%\py{For motivation of why partitioning could be useful, I suggest we show that enclave performance improves as more classes are taken out of the enclave or vice versa ie enclave perfs decrease as more classes are added to the enclave.}

\begin{figure}[!t]
	\vspace{-40pt}
	\centering
	\includegraphics[scale=0.65]{plots/motivation}
	\caption{Enclave performance is better when less classes are in the enclave.}
	\label{fig:motivation}
\end{figure}

Many real world applications may comprise sensitive portions that should be secured in an enclave. Ideally, only the secure portions should be run in the enclave, which is generally limited in terms of memory and performance. Contemporary TEE technologies like Intel SGX provide tools (\ie Intel SGX SDK) to manually partition and build enclave-based applications in native languages like C/C++, but the associated complexity has hindered the adoption of such technologies. Techniques have been proposed, \eg SCONE~\cite{scone}, Graphene-SGX~\cite{graphene}, SGX-LKL~\cite{sgxlkl} etc, which permit to easily run entire applications in enclaves. However these suffer from large TCBs which degrade application performance.

In order to motivate our work, we consider a Java application which comprises 100 classes that perform computation intensive or I/O intensive computations. We vary the number of trusted (in enclave) and untrusted (out of enclave) classes in the application, and measure the total cost of instantiating objects of each class and running their associate instance methods (computation or I/O intensive). Figure \ref{fig:motivation} shows the results obtained.

We observe that as more classes are moved out of the enclave, the overall performance of the application improves. This means by delegating some computations (which should not be secured) to the untrusted runtime, we relieve the enclave of expensive, yet insecure computations, leading to better enclave performance.

%Few research works have proposed solutions to build and partition applications into enclaves. Some works~\cite{glamdring} partition applications written in native languages (C,C++). Others~\cite{civet,uranus} propose techniques to partition managed languages like Java into enclaves. While these systems may be useful, they leverage approaches that require the presence of large LibOSes in the enclave~\cite{civet}, or require complex third party tools to assist developers in partitioning~\cite{uranus}. Furthermore, these systems lack the multi-language flexibility provided by tools such as GraalVM.

Contrary to prior work~\cite{uranus,civet}, we sought to develop a more practical (very low partitioning effort), intuitive (annotate classes), and efficient and low TCB (no LibOS) tool to assist developers in adopting security technologies such as Intel SGX for a wide range of high level languages.


